Transformer Module Networks for Systematic Generalization in Visual Question Answering

Transformers achieve great performance on Visual Question Answering (VQA). However, their systematic generalization capabilities, i.e., handling novel combinations of known concepts, is unclear. We reveal that Neural Module Networks (NMNs), i.e., question-specific compositions of modules that tackle a sub-task, achieve better or similar systematic generalization performance than the conventional Transformers, even though NMNs' modules are CNN-based. In order to address this shortcoming of Transformers with respect to NMNs, in this paper we investigate whether and how modularity can bring benefits to Transformers. Namely, we introduce Transformer Module Network (TMN), a novel NMN based on compositions of Transformer modules. TMNs achieve state-of-the-art systematic generalization performance in three VQA datasets, improving more than 30% over standard Transformers for novel compositions of sub-tasks. We show that not only the module composition but also the module specialization for each sub-task are the key of such performance gain.

==> iclr_2023/01_intro.tex <==
\section{Introduction}

%% Visual Question Answering (VQA) aims to answer questions about an image~\citep{Andreas_2016_CVPR}, and it has become the \emph{de facto} testbed to assess the capability of learning machines to perform complex visual reasoning. The compositional structure inherent to visual reasoning is at the core of  VQA---visual reasoning is a composition of visual sub-tasks, and also, visual scenes are compositions of objects, which are composed of attributes such as textures, shapes and colors. This compositional structure of VQA renders a distribution of image-question pairs of combinatorial size that cannot be fully reflected by training data. %which is of combinatorial size and cannot be comprehensively captured by training datasets. 


Visual Question Answering (VQA)~\citep{Antol_2015_ICCV} is a fundamental testbed to assess the capability of learning machines to perform complex visual reasoning. The compositional structure inherent to visual reasoning is at the core of  VQA: Visual reasoning is a composition of visual sub-tasks, and also, visual scenes are compositions of objects, which are composed of attributes such as textures, shapes and colors. This compositional structure yields a distribution of image-question pairs of combinatorial size, which cannot be fully reflected in an unbiased way by training distributions.

%% Systematic generalization is the ability to generalize to novel compositions of known concepts~\citep{lake2018generalization,bahdanau2019systematic,ruis2020benchmark}, and it is a hallmark of intelligence. A learning machine capable of systematic generalization is still a distant goal, which contrasts with the exquisite ability of current learning machines to generalize in-distribution (i.e., unseen image-question pairs from the training distribution). In fact, the most successful learning machines, i.e., Transformer-based models, have been tremendously effective for VQA when evaluated in-distribution~\citep{tan-bansal-2019-lxmert,li2019unicodervl}. \textcolor{red}{Although recent studies stressed the need to evaluate  systematic generalization instead of in-distribution generalization~\citep{gontier2020measuring,tsarkov2020cfq,bergen2021systematic}, systematic generalization capabilities of the Transformer-based models for VQA have not been investigated enough.}
% as the learning mechanisms that enable systematic generalization remain as an outstanding question at the heart of the science of intelligence, 


Systematic generalization is the ability to generalize to novel compositions of known concepts beyond the training distribution~\citep{lake2018generalization,bahdanau2019systematic,ruis2020benchmark}. A learning machine capable of systematic generalization is still a distant goal, which contrasts with the exquisite ability of current learning machines to generalize in-distribution. In fact, the most successful learning machines, i.e., Transformer-based models, have been tremendously effective for VQA when evaluated in-distribution~\citep{tan-bansal-2019-lxmert,chen2020uniter,vinvl}. Yet, recent studies stressed the need to evaluate  systematic generalization instead of in-distribution generalization~\citep{gontier2020measuring,tsarkov2020cfq,bergen2021systematic}, as the systematic generalization capabilities of Transformers for VQA are largely unknown.

%% A recent, promising strand of research investigates Neural Module Networks (NMNs) for systematic generalization in VQA~\citep{bahdanau2019systematic,closure,vanessa}. NMNs decompose a question in VQA into sub-tasks, and each sub-task is tackled with a shallow neural network called \emph{module}. Modules are composed into a question-specific network. NMNs alleviate the gap between in-distribution generalization and systematic generalization. \textcolor{red}{From our preliminary experiments, we found that a CNN-based NMN outperforms the Transformer-based models on systematic generalization to novel compositions of sub-tasks.}
%% This begs the question of whether we can improve the systematic generalization capabilities of the Transformer-based models by borrowing the NMNs’ strategies.

A recent strand of research for systematic generalization in VQA investigates Neural Module Networks (NMNs)~\citep{bahdanau2019systematic,closure,vanessa}. NMNs decompose a question in VQA into sub-tasks, and each sub-task is tackled with a shallow neural network called \emph{module}. Thus, NMNs use a question-specific composition of modules to answer novel questions. NMNs alleviate the gap between in-distribution generalization and systematic generalization due to its inherent compositional structure. In our experiments, we found that CNN-based NMNs outperform Transformers on systematic generalization to novel compositions of sub-tasks.
This begs the question of whether we can combine the strengths of Transformers and NMNs in order to improve the systematic generalization capabilities of learning machines.



% However, the current NMNs cannot rival with the Transformer-based networks, which leverage large amounts of data by using attention mechanisms that boost their overall accuracy. 


% By preliminary experiments, we found that NMNs achieve better systematic generalization performance than the Transformer-based models for novel linguistic constructs, even though they are based on convolutional neural networks (see the results on CLOSURE in Table \ref{table:results_all}).   

In this paper, we introduce \emph{Transformer Module Network (TMN)}, a novel NMN for VQA based on compositions of Transformer modules. In this way, we take the best of both worlds: the capabilities of Transformers given by attention mechanisms, and the flexibility of NMNs to adjust to questions based on novel compositions of modules. TMN allows us to investigate whether and how modularity brings benefits to Transformers in VQA. An overview of TMNs is depicted in Fig.~\ref{figure:arch}.
 
To foreshadow the results, we find that TMNs achieve state-of-the-art systematic generalization accuracy in the following three VQA datasets: CLEVR-CoGenT~\citep{clevr}, CLOSURE~\citep{closure}, and a novel test set based on GQA~\citep{gqa} that we introduce for evaluating systematic generalization performance with natural images, which we call GQA-SGL (Systematic Generalization to Linguistic combinations). Remarkably, TMNs improve systematic generalization accuracy over standard Transformers more than $30\%$ in the CLOSURE dataset, i.e., systematic generalization to novel combinations of known linguistic constructs (equivalently, sub-tasks). Our results also show that both module composition and module specialization to a sub-task are key to TMN's performance gain.
%Furthermore, our results highlight the importance of controlling the pre-training of the networks in order to ensure a fair evaluation of systematic generalization.

% In this paper, we propose \emph{Transformer Module Network (TMN)}, a novel NMN which employs Transformer encoders as a module, inspired by the high systematic generalization of modular approaches and the superior in-distribution performances of standard Transformers. Our module is a small stack of Transformer encoders. All modules have the same network structure but each module morphs into a specific module that performs a specific sub-task during training. The modules are dynamically composed into a question-specific network as in the modular approach.

% We evaluated both the standard Transformer and our Transformer Module Network in a series of experiments on three datasets: CLEVR-CoGenT \cite{clevr}, CLOSURE \cite{closure}, and our novel test set of GQA \cite{gqa_ood} designed for evaluating systematic generalization performance with natural images. We also evaluated how knowledge obtained from a large amount of pre-training data affects the performances. Our experimental results show that 1) both Transformer-based models outperform the previous state-of-the-art NMN on novel visual combinations, 2) the standard Transformer struggles with novel linguistic combinations even if we give a ground-truth task sequence, and 3) our Transformer Module Network outperforms the others on such condition.


% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.85\linewidth, clip]{figs/fig_1-2_cropped.pdf}
%     \caption{Overview of Transformer Module Network (TMN), which consists of neural modules and takes an image and a program as inputs. Each module is a small stack of Transformer encoders. The modules are dynamically taken out of a library of the modules and composed into a question-specific Transformer network. The total number of Transformer layers is the number of Transformer layers of each module $K$ $\times$ a program length $L$.   }
%     \label{figure:arch}
% \end{figure*}

\begin{figure}[!t]
    \centering
    \begin{tabular}{cc}
            \includegraphics[width=0.423\linewidth, page=1]{figs/fig_1-7_cropped.pdf}
        &   \includegraphics[width=0.517\linewidth, page=2]{figs/fig_1-7_cropped.pdf} \\
        (a) Library and module architecture & (b) Examples of question-specific networks \vspace{3mm} \\
    \end{tabular}
    \caption{\emph{Overview of Transformer Module Network (TMN)}. (a) TMN has a library of neural modules that tackle a sub-task, and each module is implemented with a small stack of Transformer encoders. (b) The modules are composed into a question-specific Transformer network. This network takes as input an image and a program that corresponds to a question. The total number of Transformer layers is the number of Transformer layers of each module ($K$) $\times$ the program length ($L$).  }
    \label{figure:arch}
\end{figure}
% The program is \{{\tt FILTER(square)}, {\tt FILTER(red)}, {\tt COUNT}\} in this example. 

% \begin{figure}[!t]
%     \centering
%     \begin{tabular}{c}
%             \includegraphics[width=0.75\linewidth, page=1]{figs/fig_1-4_cropped.pdf}\\
%              \vspace{5mm}
%         (a) Library and module architecture \\
%           \includegraphics[width=1.0\linewidth, page=2]{figs/fig_1-4_cropped.pdf} \\ \\
%         (b) Examples of question-specific networks \vspace{3mm} \\
%     \end{tabular}
%     \caption{\emph{Overview of Transformer Module Network (TMN)}. It consists of neural modules and takes as inputs an image and a program that corresponds to a question. Each module is a small stack of Transformer encoders. The modules are dynamically taken out of a library of the modules and composed into a question-specific Transformer network. The total number of Transformer layers is the number of Transformer layers of each module ($K$) $\times$ the program length ($L$).   }
%     \label{figure:arch}
% \end{figure}

==> iclr_2023/03_approach.tex <==
\section{Transformer Module Networks (TMNs)}

% \begin{figure}[!t]
%   \centering
%   \begin{minipage}[t]{0.46\textwidth}
%     \includegraphics[width=1.0\linewidth, clip]{figs/fig_2-1_cropped.pdf}
%     \caption{\emph{TMN Architecture.} Given an image and a program related to a question, TMNs firstly constructs a question-specific Transformer network with modules based on the program and extracts visual features from the image. Each module transforms representations of the visual features and a special head token with arguments. A classifier outputs an answer from the final representation of the head token.}
%     \label{figure:reasoning}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.52\textwidth}
%     \includegraphics[width=1.0\linewidth, clip]{figs/fig_3-1_cropped.pdf}
%     \caption{\emph{Stack and Tree modular structures.} Stack structure simply stacks all the modules. Tree structure runs two threads (Module 1 {$\rightarrow$} Module 2 and Module 3 $\rightarrow$ Module 4) and then merges their outputs ({\tt AND}/{\tt OR} module). \textcolor{red}{{\tt AND}/{\tt OR} module takes two sets of representations of visual features and a head token as an input and outputs the transformed representations of the first set.} (*) denotes the order of each function in the program.}
%     \label{figure:compositions}
%   \end{minipage}
% \end{figure}

\begin{figure}[!t]
  \centering
  \begin{minipage}[t]{0.38\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth, clip]{figs/fig_2-2_cropped.pdf} \\
    \vspace{1mm}
    (a) TMN Architecture
    % \label{figure:reasoning}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.54\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth, clip]{figs/fig_3-1_cropped.pdf}\\
    \vspace{1mm}
    (b) Stack and Tree modular structures
    % \label{figure:compositions}
  \end{minipage}
  \vspace{3mm}
  \caption{\emph{TMN Architecture and Modular Structures.} (a) Given an image and a program related to a question, TMNs construct a question-specific Transformer network as a composition of modules that tackle a sub-task. Each module takes as input the representations of the visual features, the head token and the module's argument from the program. A classifier outputs an answer from the final representation of the head token. (b) We investigate two modular structures. Stack structure simply stacks all the modules. Tree structure runs two threads and then merges their outputs with a module ({\tt AND}/{\tt OR} in this example). The numbers in ( ) denotes the order of each sub-task in the program.}
  \label{figure:compositions}
\end{figure}

In this section we introduce TMNs, i.e., our novel Transformer-based model for VQA that composes neural modules into a question-specific Transformer network.

%\subsection{Architecture}


\noindent {\bf Question-specific Composition of Modules.}
% \paragraph{Question-specific Composition of Modules.} 
% \subsection{Question-specific Composition of Modules}
Figure~\ref{figure:arch} provides an overview. TMNs use a library of modules, and each module tackles a different sub-task we defined (e.g., {\tt FILTER}, {\tt COUNT}). TMNs represent the question in VQA with a program, which is a sequence of sub-tasks each of which is implementable with a module from the library. 
For instance, a question ``How many red squares are there?'' can be converted to a program \{{\tt FILTER(square)}, {\tt FILTER(red)}, {\tt COUNT}\}, and then the modules corresponding to the sub-tasks are composed to form a network to answer the question.


In TMN, each module is  a stack of Transformer encoders.
Unlike the standard Transformers, which are a stack of a fixed number of Transformer encoders (typically 12) regardless of the input question, TMN composes the Transformer modules into a question-specific network, and thus, the total number of encoder layers in TMN varies according to the question.  Let $K$ be the number of Transformer encoder layers in each module, and let $L$ be the number of sub-tasks in the program. Then, TMN has a total of $K \times L$ layers to implement a program of length $L$.
%  Thus, the modules are  composed into a question-specific Transformer network. 

We follow the same approach in
previous works that directly use the program rather than the raw question~\citep{closure,bahdanau2019systematic,vanessa}. This allows to analyse systematic generalization in isolation by focusing only on visual reasoning aspects, and omits the performance of the language parser.


\noindent {\bf Transformer-based Architecture.} The aforementioned question-specific composition of modules is preceded by a feature extractor and followed by an output classifier, as shown in Fig.~\ref{figure:compositions}(a). 

We use a feature extractor to obtain the visual features of the input image. We follow the common procedure in Transformers: The visual features are transformed into the visual feature embeddings and then summed with the position embedding, which yields the input visual representations of the first module.
The initial head token representation is the average of all the visual representations. 

Then, the first Transformer module in the question-specific network takes as input the sequence of tokens consisting of the representations of the visual features, the head token, and the module's argument coming from the program. The Transformer module outputs the transformed representations of the head token and visual features. This output is fed into the next module, which also receives its corresponding argument coming from the program. Unlike Vector-NMN, whose modules always receive the initial visual representations,  in TMN only the first module receives the initial visual representations. Also, due to the versatility of Transformer architectures, in TMN we can easily change the number of Transformer encoders in each module according to the complexity of the sub-task.


Finally, a classifier outputs an answer from the final representation of the head token.


\noindent {\bf Stack and Tree Modular Structures.}
\label{subsec:modular_structures}
We further analyze the effect of modular structures.
Some modules with two inputs may be useful for constructing a network corresponding to a complex program. For instance, a logical sub-task ({\tt AND} or {\tt OR}) or sub-tasks that compare two objects. For programs containing such sub-tasks, we investigate two modular structures exemplified in Fig.~\ref{figure:compositions}(b).
The stack structure simply stacks all modules and executes the modules in sequence. The tree structure runs two threads in parallel and then merges their outputs with a module ({\tt AND}/{\tt OR} in this example), which takes two sets of representations of visual features and a head token as an input and outputs the transformed representations of the first set. We compare these two structures in the experiments. 

==> iclr_2023/04_experiments.tex <==


\section{Experimental Setup}
\label{sec:setup}

We use three datasets for VQA: two exising datasets and a novel test set we built. We compare our TMN with two Transformer-based baselines and several state-of-the-art models on those datasets.

\noindent {\bf Datasets.}
\label{subsec:dataset}
To evaluate the models for systematic generalization to novel combinations of known visual attributes or linguistic constructs, we use the following three datasets.

% \paragraph{CLEVR-CoGenT.} 
--\emph{CLEVR-CoGenT:}\quad
CLEVR is a diagnostic dataset for VQA models~\citep{clevr} that consists of  synthetic 3D scenes with multiple objects and automatically generated questions, associated with a ground-truth program formed by multiple sub-tasks.
This dataset comes with additional splits to test systematic generalization, namely, the Compositional Generalization Test (CLEVR-CoGenT). CLEVR-CoGenT is divided in two conditions where objects appear with limited color and shape combinations, that are inverted between training and testing. Using this dataset, we can test systematic generalization to novel combinations of visual attributes.

% \paragraph{CLOSURE.}
--\emph{CLOSURE:}\quad
This is a test set for models trained with CLEVR, and provides 7 benchmarks~\citep{closure}. The benchmarks test the systematic generalization to novel combinations of known linguistic constructs, which can be considered as sub-tasks, e.g., ``is the same size as'' can be a sub-task {\tt SAME$\_$SIZE}. CLOSURE uses the same synthetic images in CLEVR but contains questions which require the models to recombine the known sub-tasks in a novel way.

% since the question in VQA can be decomposed into the sub-tasks.~\citep{closure}.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=1.0\linewidth, clip]{figs/fig_4_cropped.pdf}
%     \caption{\emph{GQA-SGL test dataset for systematic generalization with natural images.} GQA-SGL is a novel test set we built based on GQA to evaluate systematic generalization performance. We generate new questions with ground-truth programs that belong to four question types (verify, query, choose, and logical) by combining the existing programs. {\textless}A,...,D{\textgreater} and {\textless}Attr{\textgreater} denote an object (e.g., chair) and an attribute (e.g., blue). {\textless}Spatial referring{\textgreater} and {\textless}Matching referring{\textgreater} are a referring expression such as `` is right of '' and `` is the same color as '', respectively.}
%     \label{figure:gqa-sgl}
% \end{figure}

% \paragraph{GQA-SGL.}
--\emph{GQA-SGL:}\quad
GQA is a VQA dataset that consists of complex natural images and questions, associated with ground-truth programs~\citep{gqa}. 
% GQA is a VQA dataset with natural images \cite{gqa}, which consists of complex natural images and questions with ground-truth programs. 
%Using the original auto-generated questions, GQA also provides balanced split, where the answer distributions are smoothed based on the program. 
GQA-SGL (Systematic Generalization to Linguistic combinations) is a novel test set we built based on GQA to test systematic generalization to novel combinations of known linguistic constructs with natural images. We generate new questions with ground-truth programs by combining the existing programs as shown in Fig.~\ref{figure:gqa-sgl} in the Appendix \ref{app:gqa_sgl}. To build the test set, we use the test-dev set from the balanced split. For the train set, in all experiments we always use the balanced split that controls bias.  See Appendix \ref{app:gqa_sgl} for details.
% a detailed description.
%for a detailed description of the dataset. 


%GQA-SGL contains 200 new questions with their program layouts. 97.4\% of the original questions can be divided into four question types: verify, query, choose, and logical. We first list out all program layouts that belong these question types, and then make a new program layout by combining the existing program, and finally generate 50 questions for each type as shown in Fig.~\ref{figure:gqa-sgl} (for details, see Appendix *).


% to prevent the model to make educated guess without understanding the images



\begin{figure}[t]
  \centering
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth, page=1]{figs/fig_5-2_cropped.pdf} \\
        \vspace{2mm}
        (a) Transformer
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth, page=2]{figs/fig_5-2_cropped.pdf} \\
        \vspace{2mm}
        (b) Transformer w/ PR
    \end{minipage}
    % \includegraphics[width=1.0\linewidth, clip]{figs/fig_2_cropped.pdf}
    % (a) Stack & (b) Tree \vspace{2mm}
    
    % \begin{tabular}{cc}
    %         \includegraphics[width=0.3\linewidth, page=1]{figs/fig_5_cropped.pdf}
    %     &   \includegraphics[width=0.3\linewidth, page=2]{figs/fig_5_cropped.pdf} \\
    %     (a) Transformer & (b) Transformer w/ PR \vspace{2mm} \\
    % \end{tabular}
    \vspace{2mm}
    \caption{\emph{Transformer-based Baseline Methods.} (a) Standard Transformer (Transformer) takes an image and a question as inputs. (b) Standard Transformer with programs (Transformer w/ PR) takes a program as an input instead of the question. {\tt Emb} denotes visual/word embeddings. These approaches use the same visual inputs and Transformer encoder structure.}
    \label{figure:models}
\end{figure}



\noindent {\bf Methods and Settings.}
\label{subsec:methods}
We compare TMNs with two Transformer-based baseline methods shown in Fig.~\ref{figure:models}. In (a), standard Transformer (Transformer) takes an image and a question as the inputs. In (b), standard Transformer with programs (Transformer w/ PR) takes a program as an input instead of the question and treat it as a sequence of tokens. TMNs also take the program as an input and executes each module with corresponding arguments as shown in Fig.~\ref{figure:compositions}. Thus, comparing Transformer w/ PR with TMNs allow us to assess the effectiveness of our Transformer modules and question-specific compositions of the modules. 
We treat VQA as a classification task and train the models with cross-entropy loss across the TMNs and our baselines.



% \noindent\paragraph{Architecture.} 
--\emph{Architecture:}\quad
We use vanilla Transformer encoder for both standard Transformers and our TMNs for fair comparison. Standard Transformers consist of 12 Transformer layers. In TMNs, the number of Transformer layers in each module is 1 for CLEVR-CoGenT and CLOSURE, and 2 for GQA-SGL because of the difference in the complexity of their sub-tasks. Transformer encoders in all models have a hidden state size of $768$ and $12$ attention heads.



% \noindent\paragraph{Library of modules and programs.} 
--\emph{Sub-tasks and programs:}\quad
For CLEVR-CoGenT and CLOSURE, we use the sub-tasks and programs defined in the dataset. For GQA-SGL, we follow the definitions proposed in \citet{mmn}.

%\noindent\paragraph{Visual features.} 
--\emph{Visual features:}\quad
For CLEVR-CoGenT and CLOSURE, we use grid features extracted by a ResNet-101 pre-trained with ImageNet to obtain the visual feature of $H \times W \times 2048$ dimensions, where $H$ and $W$ are the height and the width of the grid feature map. We add a positional encoding to the grid features and flatten them with a linear projection. We treat the flattened features as a sequence of tokens and thus the number of the tokens is $H \times W$ ($150$ on these datasets).  The input images in GQA contain various objects and are much more complex than those in CLOSURE. Therefore, for GQA-SGL, we use the popular regional features~\citep{Anderson2017up-down} extracted by a Faster R-CNN~\citep{faster_rcnn} (with a ResNet-101 backbone) pre-trained on Visual Genome dataset~\citep{visualgenome}. We consistently keep $36$ regions for each image. Each region has $2048$-dimensional visual feature and $5$-dimensional spatial location feature.

% \noindent\paragraph{Embeddings.}  
--\emph{Embeddings:}\quad
The input representation of the program is a sum of word embeddings, segment embeddings and position embeddings. They represent a sub-task or an argument (e.g., {\tt FILTER} or {\tt circle}), a thread index, and word position, respectively. For the standard Transformer, we adopt BERT tokenizer and the standard sentence embeddings described in \citep{li2019unicodervl}.

% \noindent\paragraph{Hyperparameters.} 
--\emph{Hyperparameters:}\quad
We use the Adam optimizer for all cases. Learning rates for standard Transformers and TMNs are 2e-5 and 1e-5 for CLEVR-CoGenT, 2e-5 for CLEVR, and 1e-5 and 4e-5 for GQA. We search best learning rates for each model. We train all the models with batch size of 128 on 4 Tesla V100 GPUs for 20 epochs except standard Transformer on CLEVR, 
% where we train the model for 30 epochs to converge. 
where we use 30 epochs to achieve convergence.
Training of standard Transformers and TMNs finished in 3 and 4 days, respectively. We use this experimental setup and hyperparameter tuning for all experiments.

% \noindent \paragraph{Other methods.} 
--\emph{Other methods:}\quad
We also experiment with other state-of-the-art methods, including Vector-NMN~\citep{closure}, MDETR~\citep{mdetr} and MMN~\citep{mmn} (LXMERT~\citep{tan-bansal-2019-lxmert} in Appendix \ref{sec:pretraining_appendix}). We use the hyperparamters described in the original papers. For a fair comparison, we train Vector-NMN and MMN using their publicly available code on the same training set as the rest of the methods. We also use the ground-truth programs as in TMN. MDETR was already trained on the same training set as the rest of the methods, and hence, we use the publicly available trained model. Also, we report the performance of NS-VQA~\citep{ns_vqa}   from its original paper and~\citet{akula2021robust}.

% We add several more comparison targets depending on the datasets, which  we explain in Section~\ref{Results and Analysis}. 

\section{Results and Analysis}
\label{results_and_analysis}



% We report the systematic generalization performance of the models on the following tests. In test 1 and test 2, we compare Transformer models with Vector-NMN \cite{closure}, which is a state-of-the-art neural modular network and outperforms all previous NMNs. The Vector-NMN uses the same ResNet-101 to extract the visual features from input images.
In this section, we first report the systematic generalization performance to 
% the novel visual or linguistic combinations with synthetic images (CLEVR-CoGenT and CLOSURE) 
%\textcolor{red}{the novel combinations of visual attributes or linguistic constructs (equivalently, sub-tasks) with synthetic images (CLEVR-CoGenT and CLOSURE)}
novel combinations of visual attributes or linguistic constructs with synthetic images (CLEVR-CoGenT and CLOSURE)
and complex natural images (GQA-SGL). Then, we analyze the effect of module composition, module specialization, and pre-training.
% Then, we discuss the effect of  pre-training.

\subsection{Systematic Generalization Performance}

Tables \ref{table:results_all} and \ref{table:results_gqa} show the mean and standard deviation accuracy of TMNs and the rest of approaches for both in-distribution and systematic generalization (see Appendix \ref{app:cogent}, \ref{app:closure} and \ref{app:gqa_sgl_detail} for further details). In the following, we first introduce the results in the three datasets, and then, we discuss them:

{\bf CLEVR-CoGenT.}\quad
It evaluates the systematic generalization performance to novel combinations of known visual attributes. All models are trained on CLEVR-CoGenT condition A. Our results show that both standard Transformers and TMNs largely outperform the state-of-the-art modular approaches (Vector-NMN and NS-VQA). TMNs' systematic generalization performance also surpasses  MDETR, which is the state-of-the-art Transformer-based model proposed to capture long-tail visual concepts. TMNs achieve superior performance over the standard Transformer but their performances are slightly lower than the Transformer with programs (Transformer w/ PR). As expected, Transformer w/ PR outperforms standard Transformer as the use of program facilitates visual grounding. 



% For further details about systematic generalization of these methods on the different questions of CLEVR-CoGenT B, see

% \paragraph{CLOSURE.}
{\bf CLOSURE.}\quad
It evaluates the systematic generalization performance to novel combinations of known linguistic constructs. All models are trained on CLEVR. Our results show that standard Transformers struggle with novel compositions of known linguistic constructs even when the program is provided (Transformer w/ PR).
TMNs achieve much better performance than standard Transformers and MDETR, and also outperform the other modular approaches (Vector-NMN and NS-VQA). Remarkably, TMN-Tree improves systematic generalization accuracy over standard Transformers more than $30\%$ in this dataset. Tree structure seems effective for CLOSURE because the questions often have tree structure. %See Appendix \ref{app:closure} for further details.

\begin{table}[!t]
\caption{
%\emph{Results on systematic generalization to novel visual and linguistic combinations.} 
\emph{Results on systematic generalization to novel combinations of known visual attributes and linguistic constructs.}
Mean and standard deviation of accuracy (\%) across at least three repetitions when possible (only one trained model is provided in NS-VQA and MDETR). All methods are tested on in-distribution (CLEVR-CoGenT validation condition A and CLEVR validation) and systematic generalization (CLEVR-CoGenT validation condition B and CLOSURE, indicated in yellow). We trained and test Vector-NMN on CLEVR-CoGenT in our environment while its performances on CLEVR and CLOSURE are cited from the original paper~\citep{closure}. ``Overall'' at the right end is the  mean value of accuracies on CoGenT-B and CLOSURE.}
% The performances of NS-VQA are cited from ~\citep{ns_vqa} and ~\citep{akula2021robust}.  We test MDETR using the official trained model in our environment.
\label{table:results_all}
\begin{center}
\begin{tabular}{l|l>{\columncolor[HTML]{FFFFE0}}l|l>{\columncolor[HTML]{FFFFE0}}l|c}
\multirow{3}{*}{Methods} & \multicolumn{2}{c|}{Visual attributes} & \multicolumn{2}{c|}{Linguistic constructs} &  \cellcolor[HTML]{FFFFE0} \\ \hhline{|~|-|-|-|-|~|}
                         & \multicolumn{1}{c|}{CoGenT-A} & CoGenT-B & \multicolumn{1}{c|}{CLEVR} & CLOSURE &  \multirow{-2}{*}{\cellcolor[HTML]{FFFFE0}Overall}\\
                         & \multicolumn{1}{c|}{(In-Dist.) } & (Syst. Gen.) & \multicolumn{1}{c|}{(In-Dist.)} & (Syst. Gen.) & \cellcolor[HTML]{FFFFE0}(Syst. Gen.) \\ \hline
Transformer & \multicolumn{1}{l|}{97.5 $\pm$ 0.18} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}78.9 $\pm$ 0.80}   & \multicolumn{1}{l|}{97.4 $\pm$ 0.23} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}57.4 $\pm$ 1.6} & \cellcolor[HTML]{FFFFE0}68.2 \\ %\midrule
Transformer w/ PR & \multicolumn{1}{l|}{97.4 $\pm$ 0.56} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}\textbf{81.7} $\pm$ 1.1} & \multicolumn{1}{l|}{97.1 $\pm$ 0.14} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}64.5 $\pm$ 2.5} & \cellcolor[HTML]{FFFFE0}73.1 \\ %\midrule
TMN-Stack (ours) & \multicolumn{1}{l|}{97.9 $\pm$ 0.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}80.6 $\pm$ 0.21} & \multicolumn{1}{l|}{98.0 $\pm$ 0.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}90.9 $\pm$ 0.49} & \cellcolor[HTML]{FFFFE0}85.3 \\ %\midrule
TMN-Tree (ours) & \multicolumn{1}{l|}{98.0 $\pm$ 0.02} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}80.1 $\pm$ 0.72} & \multicolumn{1}{l|}{97.9 $\pm$ 0.01} & \multicolumn{1}{l|}{\textbf{\cellcolor[HTML]{FFFFE0}95.4} $\pm$ 0.20} & \cellcolor[HTML]{FFFFE0}\textbf{87.8} \\ \hline
%Vector-NMN & \multicolumn{1}{l|}{98.0 $\pm$ 0.2} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}73.2 $\pm$ 0.2} & \multicolumn{1}{l|}{98.0 $\pm$ 0.07} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}94.4} & \cellcolor[HTML]{FFFFE0}83.8 \\ %\hline
Vector-NMN & \multicolumn{1}{l|}{98.0 $\pm$ 0.2} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}73.2 $\pm$ 0.2} & \multicolumn{1}{l|}{98.0 $\pm$ 0.07} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}94.4} & \cellcolor[HTML]{FFFFE0}83.8 \\ %\hline
NS-VQA & \multicolumn{1}{l|}{99.8} & 63.9 & \multicolumn{1}{l|}{99.8} & 76.4 & \cellcolor[HTML]{FFFFE0}70.2 \\
MDETR & \multicolumn{1}{l|}{99.7} & 76.2 & \multicolumn{1}{l|}{99.7} & 53.3 & \cellcolor[HTML]{FFFFE0}64.8
\end{tabular}
\end{center}
\end{table}

\begin{table}[!t]
\caption{\emph{Results on an application to complex natural images with novel combinations of known linguistic constructs.} Mean and standard deviation of accuracy (\%) on GQA test-dev and GQA-SGL across at least three repetitions. We use a pre-trained object detector as a feature extractor. The numbers in ( ) denote the mean accuracy on only four question types contained in GQA-SGL (verify, query, choose, and logical). Systematic generalization performance is indicated in yellow. }
\label{table:results_gqa}
\begin{center}
\begin{tabular}{l|c>{\columncolor[HTML]{FFFFE0}}c}
% \multirow{3}{*}{Methods} & \multicolumn{2}{c}{Application to natural images $^\dagger$} \\ \hhline{|~|-|-|}%\cline{2-7}
%                          & \multicolumn{1}{c|}{(In-Distribution)} & (Syst. Gen.) \\ \hline
\multirow{2}{*}{Methods} & \multicolumn{1}{c|}{GQA} & GQA-SGL \\ %\cmidrule{2-5}
                         & \multicolumn{1}{c|}{(In-Distribution)} & (Systematic generalization) \\ \hline
Transformer & \multicolumn{1}{l|}{54.9 $\pm$ 0.004 (67.6)} & 47.7 $\pm$ 2.1  \\  %\hline
Transformer w/ PR & \multicolumn{1}{l|}{54.7 $\pm$ 0.22 (67.0)} & 52.2  $\pm$ 3.2 \\ %\hline
TMN-Stack (ours) & \multicolumn{1}{l|}{52.8 $\pm$ 0.10 (64.7)} & 50.7 $\pm$ 0.94  \\ %\hline
TMN-Tree (ours) &  \multicolumn{1}{l|}{53.5 $\pm$ 0.24 (65.2)} & \textbf{53.7}  $\pm$ 1.7 \\ \hline
MMN &  \multicolumn{1}{l|}{55.6 $\pm$ 0.12 (67.8)} & 51.0  $\pm$ 1.5
\end{tabular}
\end{center}
\end{table}

% In Table \ref{table:closure_details} in Appendix, we report the performance across the different question constructs in CLOSURE. 

%\subsection{Application to Natural Images}

% We apply our models on complex natural images. With GQA-SGL, we evaluate the systematic generalization performance to novel linguistic combinations with natural images. 
%\paragraph{GQA-SGL.} 
{\bf GQA-SGL.}\quad
We evaluate the systematic generalization performance to novel combinations of known linguistic constructs with natural images. All models are trained on GQA. In Table \ref{table:results_gqa}, we evaluate the exact matching between the predicted and  ground-truth answers, on both GQA and GQA-SGL.  TMN-Tree achieves superior performance on systematic generalization with a smaller drop of in-distribution accuracy compared to standard Transformers. Although MMN is the recently proposed NMN for GQA and achieves great in-distribution performance, TMN-Tree outperforms MMN on systematic generalization.

%\paragraph{Effectiveness of modularity.} 
% {\bf Effectiveness of dynamic composition of modules.}\quad
{\bf Discussion of the Results.}\quad
Our results in CLOSURE and GQA-SGL show that TMNs (i.e., introducing modularity to Transformers) improve the systematic generalization performance to novel combinations of known linguistic constructs (i.e., novel compositions of sub-tasks) of Transformers and NMNs. The performance gain in CLOSURE is relatively larger than that in GQA-SGL tests. One reason to explain this is the complexity of the questions: the maximum program length is $26$ in CLOSURE, while it is $9$ in GQA. CLOSURE provides more complex questions which require stronger systematic generalization capabilities.  Results in CLEVR-CoGenT show that TMNs do not improve systematic generalization of Transformers for novel compositions of visual attributes. This may be expected as the visual feature extractor is the key component for generalization to novel combinations of visual attributes~\citep{vanessa}, and Transformer and TMNs have the same visual feature extractor.
Finally, we observe that TMNs achieve the best accuracy across all tested methods in CLOSURE and GQA-SGL, and competitive accuracy with the best performing method in CLEVR-CoGenT. 

%SOA (compare against the rest)


%In other words, modularity can benefit Transformer-based model to operate novel combinations of known sub-tasks by  composing modules, while standard Transformers struggle with operating the novel combinations of the sub-tasks by a fixed number of encoder layers.


%but not for the novel visual combinations. ...



\begin{table}[!t]
\caption{\emph{Effect of specialization of modules.} Mean and standard deviation of accuracy (\%) on CLEVR and CLOSURE across three repetitions with different libraries of modules. 
``Individual'' denotes that a module is assigned to a single sub-task. ``Semantic group'' and ``Random group'' denote that a module is assigned to a group including sub-tasks that are semantically similar or randomly selected, respectively. ``Order'' denotes that a module is selected by the order of a sub-task in a program.
}
\label{table:results_modularity}
\begin{center}
\begin{tabular}{l|c|c|cc}
Library & The number & Specialization & \multicolumn{1}{c|}{CLEVR} & CLOSURE \\ %\cmidrule{2-5}
                        of modules & of modules & of modules & \multicolumn{1}{c|}{(In-Distribution)} & (Syst. Generalization) \\ \hline
Individual & 26 & $\checkmark$ & \multicolumn{1}{l|}{98.0 $\pm$ 0.030} & 90.9 $\pm$ 0.49  \\
Semantic group & 12 & $\checkmark$ & \multicolumn{1}{l|}{98.1 $\pm$ 0.014} & \textbf{93.7  $\pm$ 0.55} \\ 
Random group & 12 & $\checkmark$ & \multicolumn{1}{l|}{97.9 $\pm$ 0.059} & 93.0  $\pm$ 0.29 \\ 
Order & 12 & & \multicolumn{1}{l|}{92.2 $\pm$ 1.5} & 68.4 $\pm$ 1.8   \\
\end{tabular}
\end{center}
\end{table}

%\input{neurips_2022/tabletest1}

\begin{table}[!t]
\caption{\emph{Ablation analysis.} Mean and standard deviation of accuracy (\%) on CLEVR and CLOSURE across three repetitions. We add imitations of properties of TMN, i.e., Variable number of  layers (VL) and Split tokens (ST) to the standard Transformer w/ PR. SoM stands for the specialization of the modules.}
% VL is an imitation of the question-specific composition of modules in TMN and changes the number of layers depending on a program length (up to $26$), but the each layer (module in TMN) is not specialized for specific sub-tasks. 
\label{table:results_ablation}
\begin{center}
\begin{tabular}{l|c|c|c|c|c}
\multirow{2}{*}{Methods} &\multicolumn{3}{c|}{Properties} & CLEVR & CLOSURE \\ \hhline{|~|-|-|-|~|~|}
 & VL & ST & SoM & (In-Distribution) & (Syst. Generalization) \\ \hline
Transformer w/ PR & & & & \multicolumn{1}{l|}{97.1 $\pm$ 0.14} & 64.5 $\pm$ 2.5  \\
% Transformer w/ PR + DL & $\checkmark$ & & &\multicolumn{1}{l|}{97.0 $\pm$ 0.32} & 60.4  $\pm$ 2.7 \\
Transformer w/ PR + VL & $\checkmark$ & & &\multicolumn{1}{l|}{94.0 $\pm$ 1.8} & 60.2  $\pm$ 2.9 \\ 
% Transformer w/ PR + DL + ST& $\checkmark$ & $\checkmark$ &  & \multicolumn{1}{l|}{59.3 $\pm$ 0.50} &
Transformer w/ PR + VL + ST& $\checkmark$ & $\checkmark$ &  & \multicolumn{1}{l|}{56.8 $\pm$ 0.042} & 43.6 $\pm$ 0.59  \\
TMN-Stack & $\checkmark$ & $\checkmark$ & $\checkmark$ & \multicolumn{1}{l|}{98.0 $\pm$ 0.030} & \textbf{90.9 $\pm$ 0.49}   \\
\end{tabular}
\end{center}
\end{table}
%\input{neurips_2022/tabletest2}

\subsection{Analysis} %Effect of Specialization of Modules}

\noindent
{\bf Module Behaviors.}\quad
We analyze the behavior of our trained modules, i.e.,  how Transformer modules work, by visualizing attention maps. See Fig. \ref{figure:attentiom_map} in Appendix \ref{app:visualize}. The qualitative results indicate that the modules learn their functions properly.

%\paragraph{Module Specialization.} 
\noindent
{\bf  Module Specialization.}\quad
While the question-specific composition of modules is a key property of NMNs, a recent work reports that a degree of modularity of the NMN also has large influence on systematic generalization \citep{vanessa}. Here we also investigate this aspect for TMNs. 
%how the degree of modularity affects the systematic generalization performance of the TMN-Stack. 
Table \ref{table:results_modularity} shows the mean accuracy of TMN-Stack with four different libraries of modules, each with a different degree of specialization.
``Individual'' denotes that each module is assigned to a single sub-task ($26$ sub-tasks defined in CLEVR in total). This is the library used in the previous sections. 
``Semantic group'' denotes that each module tackles a group of sub-tasks that are semantically similar. %(e.g., {\tt FILTER\_COLOR}, {\tt FILTER\_SIZE}, ...). 
``Random group'' denotes that each module tackles  a group of sub-tasks randomly selected. % (e.g., {\tt FILTER\_COLOR}, {\tt COUNT}, ...). 
``Order'' denotes that each module is always placed in the same position of the question-specific network, independently of the sub-task performed in that position. If there are more sub-tasks in the program than modules in the library, the modules are repeated following the same order. In this way, we compare the importance of modules tackling sub-tasks with the importance of having a question-specific network.  See Appendix \ref{sec:libraries_appendix} for further details about each library. 
% All libraries are trained for 20 epochs on CLEVR dataset.

Results shows that the systematic generalization accuracy largely drops when the modules are not specialized, even if the number of modules is the same (compare ``Order'' with ``Semantic group'' and ``Random group''). The degree of modularity (Individual vs Semantic group) and how sub-tasks are grouped (Semantic vs Random) also affects the systematic generalization performance. These results suggest that question-specific composition of modules is not enough and specialization of modules is crucially important. 
Finally, note that the results of Semantic group and Random group also show that TMN performs better than the standard Transformer ($93.7$ vs $64.5$) even if the total number of parameters that all modules have is the same as the number of parameters of the standard Transformer (i.e., TMN has $12$ modules of one layer each, while Transformers have $12$ layers).

\noindent
{\bf Ablation Analysis.}
We investigate the contribution of TMN's  specialization of modules (SoM) to TMNs' superior performance over standard Transformer. %To do so, we add imitations of properties of TMN, i.e., Variable number of layers (VL) and Split tokens (ST) to the standard Transformer w/ PR. These are introduced in the following and then we report the results.
Besides SoM, TMNs also have a variable number of layers, while  standard Transformer have a fixed number of layers. We analyze if it is this difference in number of layers or the SoM that is causing TMNs' higher accuracy. To do so, we add a property named Variable number of layers (VL) to the Transformer w/ PR. With the VL, the Transformer w/ PR uses as many encoder layers as the program length (e.g., 18 layers are used to output an answer for an input program with a length of 18). VL can be regarded as an imitation of the question-specific  compositions of the modules in TMN, but each layer is not specialized for  specific sub-tasks. 
Another key difference between TMNs and Transformers besides SoM is that TMN modules takes as  argument tokens related to the sub-task as indicated by the program, while every layer of standard Transformer takes all input tokens in the program, because Transformers' layers are not specialized to sub-tasks. Splitting the program tokens may help the model to steer the computations that should be executed at each layer. To investigate this, we add this property, named as Split Tokens (ST), to the Transformer w/ PR.

Table \ref{table:results_ablation} shows that any of the aforementioned properties do not improve the systematic generalization performance without the specialization of modules to sub-tasks, i.e., SoM. 
% , where all methods are trained for 20 epochs with CLEVR dataset. 
Even with Split tokens, the performance does not improve because the layers can not be specialized and splitting the token can spoil the flexibly of the standard Transformer.

%All methods are trained for 20 epochs with CLEVR dataset. 

% Dynamic layers is a imitation of dynamic composition of TMN, but each layers are not specialized for the specific sub-task like Order in \ref{table:results_modularity}. This could be a reason not to show the performance improvement. Even With Split tokens, the performance does not improve because the layers can not be specialized.

% Dynamic layers is a imitation of dynamic composition of TMN, but each layers are not specialized for the specific sub-task like Order in \ref{table:results_modularity}. This could be a reason not to show the performance improvement. 
% We add imitations of features of TMN to standard Transformer w/ PR to analyze the components of TMN, i.e., Dynamic layers and Split tokens. 



% Just write down:
% \begin{enumerate}
%   \item Modules are designed by human not automatically, self-modularization, self-supervised learning with large amount of data
%   \item Need programs or decomposing questions into sub-tasks (modules), or difficulty to apply to other datasets/tasks without programs
%   \item The number of layers of module are constant across all modules and it is practically decided, the number of layers can be optimized for each module
% \end{enumerate}

\begin{table}[!t]
\caption{\emph{Effect of pre-training.} Mean accuracy (\%) on CLEVR-CoGenT validation condition B and CLOSURE with two different feature extractors, which are an object detector pre-trained on Visual Genome (VG) and a ResNet-101 (without pre-training on VG).} 
\label{table:cogent_pretrain}
\begin{center}
\begin{tabular}{l|c|c|c|c|c|c}
\multirow{2}{*}{Methods} & \multicolumn{3}{c|}{CLEVR-CoGenT} & \multicolumn{3}{c}{CLOSURE}  \\ \hhline{|~|-|-|-|-|-|-|}
& w/o VG & w/ VG & $\Delta$ & w/o VG & w/ VG & $\Delta$ \\ \hline
Transformer & 78.9 & 87.5 & 8.6 & 57.4 & 62.1 & 4.7 \\  %\hline
Transformer w/ PR & \textbf{81.7} & \textbf{88.7} & 6.9 & 64.5 & 64.5 & 0.005  \\  %\hline 
TMN-Stack (ours) & 80.6 & 86.9 & 6.3 & 90.9 & 92.7 & 1.7 \\  %\hline
TMN-Tree (ours) & 80.1 & 86.4 & 6.4 & \textbf{95.4} & \textbf{96.4} & 1.0    \\
\end{tabular}
\end{center}
\end{table}

% \paragraph{Pre-training.}Furthermore, we investigate the effect of the pre-training of the networks and carefully control it in order to ensure a fair evaluation of systematic generalization. See Appendix \ref{sec:pretraining_appendix} for further details.

%\paragraph{Pre-training.} 
\noindent
{\bf Pre-training.}\quad
We analyze how the additional image data from other domains affects systematic generalization to novel combinations of visual attributes or linguistic constructs, i.e., CLEVR-CoGenT and CLOSURE, respectively. Table \ref{table:cogent_pretrain} shows the mean accuracy with two different visual features, namely, regional features extracted by an object detector pre-trained on Visual Genome (VG) and grid features extracted by a ResNet-101 without pre-training on VG. Across all the tested models, we observe, as expected, that the performance gains from pre-training the visual feature extractor are  larger  for generalization to novel visual combinations and smaller for novel linguistic combinations.  
This highlights the need to control  pre-training in order to ensure a fair comparison of different methods for systematic generalization.
See Appendix \ref{sec:regional_appendix} and \ref{sec:pretraining_appendix} for further experiments.

==> iclr_2023/06_code_and_data_availability.tex <==
%\paragraph{Code and data availability statement.} 

\noindent
{\bf Code and data availability statement.}\quad
The code and new dataset used in this study is included in the supplementary materials and will be made publicly available upon acceptance.

==> iclr_2023/07_acknowledgement.tex <==
\section*{Acknowledgements and Disclosure of Funding} 
We would like to thank Pawan Sinha, Serban Georgescu, Hisanao Akima and Tomaso Poggio for warm encouragement and insightful advice. 
This work has been supported by Fujitsu Limited (Contract No. 40009105 and 40009568) and by the Center for Brains, Minds and Machines (funded by NSF STC award CCF-1231216). 
XB is supported by the R01EY020517 grant from the National Eye Institute (NIH). 

==> iclr_2023/08_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

\begin{enumerate}
   \item Modules are designed by human not automatically, self-modularization, self-supervised learning with large amount of data
   \item Need programs or decomposing questions into sub-tasks (modules), or difficulty to apply to other datasets/tasks without programs
   \item The number of layers of module are constant across all modules and it is practically decided, the number of layers can be optimized for each module
\end{enumerate}

==> neurips_2022_rebuttal/00_abstract.tex <==
Transformer-based models achieve great performance on Visual Question Answering (VQA). However, their systematic generalization capabilities, i.e., handling novel combinations of known concepts, is unclear.
We reveal that neural networks that compose modules that tackle sub-tasks (i.e., Neural Module Networks, NMNs) achieve {\color{blue} in some cases} better systematic generalization performance than the {\color{blue} conventional} Transformer-based models, even though NMNs are CNN-based. To investigate whether and how modularity brings benefits to Transformer-based models, we propose Transformer Module Network (TMN), a novel Transformer-based model for VQA that composes Transformer modules into a question-specific network. 
TMNs achieve state-of-the-art systematic generalization performance in three VQA datasets, improving more than $30\%$ over standard Transformers for the novel compositions of the sub-tasks.
We also show that not only the module composition but also the module specialization for each sub-task is the key of the performance gain.

==> neurips_2022_rebuttal/04_experiments.tex <==


\section{Experimental Setup}
\label{sec:setup}

We use three datasets for VQA: two exising datasets and a novel test set we built. We compare our TMN with two Transformer-based baselines and several state-of-the-art models on those datasets.

\noindent {\bf Datasets.}
\label{subsec:dataset}
To evaluate the models for systematic generalization to novel combinations of known visual attributes or linguistic constructs, we use the following three datasets.

% \paragraph{CLEVR-CoGenT.} 
--\emph{CLEVR-CoGenT:}\quad
CLEVR is a diagnostic dataset for VQA models~\citep{clevr} that consists of  synthetic 3D scenes with multiple objects and automatically generated questions, associated with a ground-truth program formed by multiple sub-tasks.
This dataset comes with additional splits to test systematic generalization, namely, the Compositional Generalization Test (CLEVR-CoGenT). CLEVR-CoGenT is divided in two conditions where objects appear with limited color and shape combinations, that are inverted between training and testing. Using this dataset, we can test systematic generalization to novel combinations of visual attributes.

% \paragraph{CLOSURE.}
--\emph{CLOSURE:}\quad
This is a test set for models trained with CLEVR, and provides 7 benchmarks~\citep{closure}. The benchmarks test the systematic generalization to novel combinations of known linguistic constructs, which can be considered as sub-tasks, e.g., ``is the same size as'' can be a sub-task {\tt SAME$\_$SIZE}. CLOSURE uses the same synthetic images in CLEVR but contains questions which require the models to recombine the known sub-tasks in a novel way.

% since the question in VQA can be decomposed into the sub-tasks.~\citep{closure}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth, clip]{figs/fig_4_cropped.pdf}
    \caption{\emph{GQA-SGL test dataset for systematic generalization with natural images.} GQA-SGL is a novel test set we built based on GQA to evaluate systematic generalization performance. We generate new questions with ground-truth programs that belong to four question types (verify, query, choose, and logical) by combining the existing programs. {\textless}A,...,D{\textgreater} and {\textless}Attr{\textgreater} denote an object (e.g., chair) and an attribute (e.g., blue). {\textless}Spatial referring{\textgreater} and {\textless}Matching referring{\textgreater} are a referring expression such as `` is right of '' and `` is the same color as '', respectively.}
    \label{figure:gqa-sgl}
\end{figure}

% \paragraph{GQA-SGL.}
--\emph{GQA-SGL:}\quad
GQA is a VQA dataset that consists of complex natural images and questions, associated with ground-truth programs~\citep{gqa}. 
% GQA is a VQA dataset with natural images \cite{gqa}, which consists of complex natural images and questions with ground-truth programs. 
%Using the original auto-generated questions, GQA also provides balanced split, where the answer distributions are smoothed based on the program. 
GQA-SGL (Systematic Generalization to Linguistic combinations) is a novel test set we built based on GQA to test systematic generalization to novel combinations of known linguistic constructs with natural images. We generate new questions with ground-truth programs by combining the existing programs as shown in Fig.~\ref{figure:gqa-sgl}. We only use test-dev balanced split to build this test set, and in all experiments with GQA, we always use the balanced split that controls bias.  See Appendix \ref{app:gqa_sgl} for a detailed description.
%for a detailed description of the dataset. 


%GQA-SGL contains 200 new questions with their program layouts. 97.4\% of the original questions can be divided into four question types: verify, query, choose, and logical. We first list out all program layouts that belong these question types, and then make a new program layout by combining the existing program, and finally generate 50 questions for each type as shown in Fig.~\ref{figure:gqa-sgl} (for details, see Appendix *).


% to prevent the model to make educated guess without understanding the images





\noindent {\bf Methods and Settings.}
\label{subsec:methods}
We compare TMNs with two Transformer-based baseline methods shown in Fig.~\ref{figure:models}. In (a), standard Transformer (Transformer) takes an image and a question as the inputs. In (b), standard Transformer with programs (Transformer w/ PR) takes a program as an input instead of the question and treat it as a sequence of tokens. TMNs also take the program as an input and executes each module with corresponding arguments as shown in Fig.~\ref{figure:compositions}. Thus, comparing Transformer w/ PR with TMNs allow us to assess the effectiveness of our Transformer modules and question-specific compositions of the modules. 




% \noindent\paragraph{Architecture.} 
--\emph{Architecture:}\quad
We use vanilla Transformer encoder for both standard Transformers and our TMNs for fair comparison. Standard Transformers consist of 12 Transformer layers. In TMNs, the number of Transformer layers in each module is 1 for CLEVR-CoGenT and CLOSURE, and 2 for GQA-SGL because of the difference in the complexity of their sub-tasks. Transformer encoders in all models have a hidden state size of $768$ and $12$ attention heads.



% \noindent\paragraph{Library of modules and programs.} 
--\emph{Sub-tasks and programs:}\quad
For CLEVR-CoGenT and CLOSURE, we use the sub-tasks and programs defined in the dataset. For GQA-SGL, we follow the definitions proposed in \citep{mmn}.

%\noindent\paragraph{Visual features.} 
--\emph{Visual features:}\quad
For CLEVR-CoGenT and CLOSURE, we use grid features extracted by a ResNet-101 pre-trained with ImageNet to obtain the visual feature of $H \times W \times 2048$ dimensions, where $H$ and $W$ are the height and the width of the grid feature map. We add a positional encoding to the grid features and flatten them with a linear projection. We treat the flattened features as a sequence of tokens and thus the number of the tokens is $H \times W$ ($150$ on these datasets).  The input images in GQA contain various objects and are much more complex than those in CLOSURE. Therefore, for GQA-SGL, we use popular regional features~\citep{Anderson2017up-down} extracted by a Faster R-CNN~\citep{faster_rcnn} (with a ResNet-101 backbone) pre-trained on Visual Genome dataset~\citep{visualgenome}. We consistently keep $36$ regions for each image. Each region has $2048$-dimensional visual feature and $5$-dimensional spatial location feature.

% \noindent\paragraph{Embeddings.}  
--\emph{Embeddings:}\quad
Input representation of the program is sum of word embeddings, segment embeddings and position embeddings. They represent a sub-task or an argument (e.g., {\tt FILTER} or {\tt circle}), a thread index, and word position, respectively. For the standard Transformer, we adopt BERT tokenizer and a standard sentence embeddings described in \citep{li2019unicodervl}.

% \noindent\paragraph{Hyperparameters.} 
--\emph{Hyperparameters:}\quad
We use the Adam optimizer for all the cases. Learning rates for standard Transformers and TMNs are 2e-5 and 1e-5 for CLEVR-CoGenT, 2e-5 for CLEVR, and 1e-5 and 4e-5 for GQA. We search best learning rates for each model. We train all the models with batch size of 128 on 4 Tesla V100 GPUs for 20 epochs except standard Transformer on CLEVR, 
% where we train the model for 30 epochs to converge. 
where we use 30 epochs to achieve convergence.
Training of standard Transformers and TMNs finished in 3 and 4 days, respectively. We use this experimental setup and hyperparameter tuning for all experiments.

% \noindent \paragraph{Other methods.} 
--\emph{Other methods:}\quad
We also experiment with other state-of-the-art methods, including Vector-NMN~\citep{closure} and MDETR~\citep{mdetr} (LXMERT~\citep{tan-bansal-2019-lxmert} and MMN~\citep{mmn} in Appendix \ref{sec:pretraining_appendix}). We follow the parameters described in the original papers. {\color{blue} We also cite the performance of NS-VQA~\citep{ns_vqa}  from its original paper and \citep{akula2021robust}. }

% We add several more comparison targets depending on the datasets, which  we explain in Section~\ref{Results and Analysis}. 


\begin{figure}[t]
  \centering
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=0.6\linewidth, page=1]{figs/fig_5_cropped.pdf} \\
        \vspace{2mm}
        (a) Transformer
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=0.6\linewidth, page=2]{figs/fig_5_cropped.pdf} \\
        \vspace{2mm}
        (b) Transformer w/ PR
    \end{minipage}
    % \includegraphics[width=1.0\linewidth, clip]{figs/fig_2_cropped.pdf}
    % (a) Stack & (b) Tree \vspace{2mm}
    
    % \begin{tabular}{cc}
    %         \includegraphics[width=0.3\linewidth, page=1]{figs/fig_5_cropped.pdf}
    %     &   \includegraphics[width=0.3\linewidth, page=2]{figs/fig_5_cropped.pdf} \\
    %     (a) Transformer & (b) Transformer w/ PR \vspace{2mm} \\
    % \end{tabular}
    \vspace{2mm}
    \caption{\emph{Transformer-based baseline methods.} (a) Standard Transformer (Transformer) takes an image and a question as inputs. (b) Standard Transformer with programs (Transformer w/ PR) takes a program as an input instead of the question. Visual inputs and the Transformer encoder layers are exactly the same.}
    \label{figure:models}
\end{figure}

\section{Results and Analysis}
\label{results_and_analysis}



% We report the systematic generalization performance of the models on the following tests. In test 1 and test 2, we compare Transformer models with Vector-NMN \cite{closure}, which is a state-of-the-art neural modular network and outperforms all previous NMNs. The Vector-NMN uses the same ResNet-101 to extract the visual features from input images.
We report the systematic generalization performance to 
% the novel visual or linguistic combinations with synthetic images (CLEVR-CoGenT and CLOSURE) 
%\textcolor{red}{the novel combinations of visual attributes or linguistic constructs (equivalently, sub-tasks) with synthetic images (CLEVR-CoGenT and CLOSURE)}
the novel combinations of visual attributes or linguistic constructs with synthetic images (CLEVR-CoGenT and CLOSURE)
and complex natural images (GQA-SGL). Then, we analyze the effect of module composition, module specialization, and pre-training.
% Then, we discuss the effect of  pre-training.

\subsection{Systematic Generalization Performance}

Tables \ref{table:results_all} and \ref{table:results_gqa} show the mean and standard deviation accuracy of TMNs and rest of approaches for both in-distribution and systematic generalization (see Appendix \ref{app:cogent}, \ref{app:closure} and \ref{app:gqa_sgl_detail} for further details). In the following, we first introduce the results in the three datasets, and then, we discuss them:

{\bf CLEVR-CoGenT.}\quad
With CLEVR-CoGenT, we evaluate the systematic generalization performance to novel combinations of known visual attributes. All models are trained on CLEVR-CoGenT condition A. Our results show that both standard Transformers and TMNs largely outperform the state-of-the-art NMN (Vector-NMN~\citep{closure}). TMNs' systematic generalization performance also surpasses  MDETR~\citep{mdetr}, which is the state-of-the-art Transformer-based model proposed to capture long-tail visual concepts. TMNs achieve superior performance over the standard Transformer but their performances are slightly lower than the Transformer with programs. As expected, Transformer w/ PR outperforms standard Transformer as the use of program facilitates visual grounding. %See Appendix \ref{app:cogent} for further details.



% For further details about systematic generalization of these methods on the different questions of CLEVR-CoGenT B, see

% \paragraph{CLOSURE.}
{\bf CLOSURE.}\quad
With CLOSURE, we evaluate the systematic generalization performance to novel combinations of known linguistic constructs. All the models are trained on CLEVR. Our results show that standard Transformers struggle with the novel compositions of known linguistic constructs even when the program is provided (Transformer w/ PR).
Our TMNs achieve much better performance than the standard Transformers, and also outperform the Vector-NMN. Remarkably, TMN-Tree improves systematic generalization accuracy over standard Transformers more than $30\%$ in this dataset. Tree structure seems effective for CLOSURE because the questions often have tree structure. %See Appendix \ref{app:closure} for further details.

\begin{table}[!t]
\caption{
%\emph{Results on systematic generalization to novel visual and linguistic combinations.} 
\emph{Results on systematic generalization to novel combinations of known visual attributes and linguistic constructs.}
Mean and standard deviation of accuracy (\%) across at least three repetitions. All methods are tested on in-distribution (CLEVR-CoGenT validation condition A and CLEVR validation) and systematic generalization (CLEVR-CoGenT validation condition B and CLOSURE, indicated in yellow). We trained and test Vector-NMN on CLEVR-CoGenT in our environment while its performances on CLEVR and CLOSURE are cited from the original paper~\citep{closure}. {\color{blue} The performances of NS-VQA are cited from ~\citep{ns_vqa} and ~\citep{akula2021robust}.}  We test MDETR using the official trained model in our environment. ``Overall'' at the right end is the  mean value of accuracies on CoGenT-B and CLOSURE.}
\label{table:results_all}
\centering
\begin{tabular}{l|l>{\columncolor[HTML]{FFFFE0}}l|l>{\columncolor[HTML]{FFFFE0}}l|c}
\toprule
% \hline
\multirow{3}{*}{Methods} & \multicolumn{2}{c|}{Visual attributes} & \multicolumn{2}{c|}{Linguistic constructs} &  \\ \cmidrule{2-5}%\hhline{|~|-|-|-|-|} %\cline{2-7}
                         & \multicolumn{1}{c|}{CoGenT-A} & CoGenT-B & \multicolumn{1}{c|}{CLEVR} & CLOSURE & \cellcolor[HTML]{FFFFE0}Overall   \\
                         & \multicolumn{1}{c|}{(In-Dist.) } & (Syst. Gen.) & \multicolumn{1}{c|}{(In-Dist.)} & (Syst. Gen.) & \cellcolor[HTML]{FFFFE0}(Syst. Gen.) \\ \midrule
Transformer & \multicolumn{1}{l|}{97.5 $\pm$ 0.18} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}78.9 $\pm$ 0.80}   & \multicolumn{1}{l|}{97.4 $\pm$ 0.23} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}57.4 $\pm$ 1.6} & \cellcolor[HTML]{FFFFE0}68.2 \\ %\midrule
Transformer w/ PR & \multicolumn{1}{l|}{97.4 $\pm$ 0.56} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}\textbf{81.7} $\pm$ 1.1} & \multicolumn{1}{l|}{97.1 $\pm$ 0.14} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}64.5 $\pm$ 2.5} & \cellcolor[HTML]{FFFFE0}73.1 \\ %\midrule
TMN-Stack (ours) & \multicolumn{1}{l|}{97.9 $\pm$ 0.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}80.6 $\pm$ 0.21} & \multicolumn{1}{l|}{98.0 $\pm$ 0.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}90.9 $\pm$ 0.49} & \cellcolor[HTML]{FFFFE0}85.3 \\ %\midrule
TMN-Tree (ours) & \multicolumn{1}{l|}{98.0 $\pm$ 0.02} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}80.1 $\pm$ 0.72} & \multicolumn{1}{l|}{97.9 $\pm$ 0.01} & \multicolumn{1}{l|}{\textbf{\cellcolor[HTML]{FFFFE0}95.4} $\pm$ 0.20} & \cellcolor[HTML]{FFFFE0}\textbf{87.8} \\ %\midrule
Vector-NMN & \multicolumn{1}{l|}{98.0 $\pm$ 0.2} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}73.2 $\pm$ 0.2} & \multicolumn{1}{l|}{98.0 $\pm$ 0.07} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFE0}94.4} & \cellcolor[HTML]{FFFFE0}83.8 \\ \midrule
\color{blue}{NS-VQA} & \multicolumn{1}{l|}{\color{blue}{99.8}} & \cellcolor[HTML]{FFFFFF}\color{blue}{63.9} & \multicolumn{1}{l|}{\color{blue}{99.8}} & \cellcolor[HTML]{FFFFFF}\color{blue}{76.4} & \color{blue}{70.2} \\
MDETR & \multicolumn{1}{l|}{99.7} & \cellcolor[HTML]{FFFFFF}76.2 & \multicolumn{1}{l|}{99.7} & \cellcolor[HTML]{FFFFFF}53.3 & 64.8 \\ %\hline
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!t]
\caption{\emph{Results on an application to complex natural images with novel combinations of known linguistic constructs.} Mean and standard deviation of accuracy (\%) on GQA test-dev and GQA-SGL across at least three repetitions. We use a pre-trained object detector as a feature extractor. The numbers in ( ) denote the mean accuracy on only four question types contained in GQA-SGL (verify, query, choose, and logical). Systematic generalization performance is indicated in yellow.}
\label{table:results_gqa}
\centering
\begin{tabular}{l|c>{\columncolor[HTML]{FFFFE0}}c}
\toprule
% \multirow{3}{*}{Methods} & \multicolumn{2}{c}{Application to natural images $^\dagger$} \\ \hhline{|~|-|-|}%\cline{2-7}
%                          & \multicolumn{1}{c|}{(In-Distribution)} & (Syst. Gen.) \\ \hline
\multirow{2}{*}{Methods} & \multicolumn{1}{c|}{GQA} & GQA-SGL \\ %\cmidrule{2-5}
                         & \multicolumn{1}{c|}{(In-Distribution)} & (Systematic generalization) \\ \midrule %\hline
Transformer & \multicolumn{1}{l|}{54.9 $\pm$ 0.004 (67.6)} & 47.7 $\pm$ 2.1  \\  %\hline
Transformer w/ PR & \multicolumn{1}{l|}{54.7 $\pm$ 0.22 (67.0)} & 52.2  $\pm$ 3.2 \\ %\hline
TMN-Stack (ours) & \multicolumn{1}{l|}{52.8 $\pm$ 0.10 (64.7)} & 50.7 $\pm$ 0.94  \\ %\hline
TMN-Tree (ours) &  \multicolumn{1}{l|}{53.5 $\pm$ 0.24 (65.2)} & \textbf{53.7}  $\pm$ 1.7 \\ \bottomrule
\end{tabular}
\end{table}

% In Table \ref{table:closure_details} in Appendix, we report the performance across the different question constructs in CLOSURE. 

%\subsection{Application to Natural Images}

% We apply our models on complex natural images. With GQA-SGL, we evaluate the systematic generalization performance to novel linguistic combinations with natural images. 
%\paragraph{GQA-SGL.} 
{\bf GQA-SGL.}\quad
With GQA-SGL, we evaluate the systematic generalization performance to novel combinations of known linguistic constructs with natural images. All the models are trained on GQA. In Table \ref{table:results_gqa}, we evaluate the exact matching between the predicted and  ground-truth answers, on both GQA and GQA-SGL.  The TMN-Tree achieves superior performance on systematic generalization with a smaller drop from the in-distribution accuracy compared to the standard Transformers. %See Appendix \ref{app:gqa_sgl_detail} for further details.

%\paragraph{Effectiveness of modularity.} 
% {\bf Effectiveness of dynamic composition of modules.}\quad
{\bf Discussion of the Results.}\quad
In the series of experiments on three VQA datasets, our results reveal that introducing modularity to Transformer improves the systematic generalization performance to the novel combinations of known linguistic constructs, or equivalently, sub-tasks (CLOSURE and GQA-SGL). The performance gain in CLOSURE is relatively larger than that in GQA-SGL tests. One reason could be the complexity of the questions. The maximum program length is $26$ in CLOSURE, while it is $9$ in GQA. CLOSURE provides more complex questions which require stronger systematic generalization capabilities.  

The results also show that introducing modularity to Transformer does not improve systematic generalization for novel compositions of visual attributes (CLEVR-CoGenT). This may be expected as the visual feature extractor is the key component for generalization to novel combinations of visual attributes~\citep{vanessa}, and Transformer and TMNs have the same visual feature extractor.


%the visual feature extractor is pre-trained in ImageNet and its weights are frozen during training in CoGenT. The features learned in ImageNet may provide a visual feature that can be leveraged to recognize novel combinations of visual attributes from CoGenT.


Finally, we observe that TMNs achieve the best accuracy across all tested methods in CLOSURE and GQA-SGL, and competitive accuracy with the best performing method in CLEVR-CoGenT. 

%SOA (compare against the rest)


%In other words, modularity can benefit Transformer-based model to operate novel combinations of known sub-tasks by  composing modules, while standard Transformers struggle with operating the novel combinations of the sub-tasks by a fixed number of encoder layers.


%but not for the novel visual combinations. ...



\begin{table}[!t]
\caption{\emph{Effect of specialization of modules.} Mean and standard deviation of accuracy (\%) on CLEVR and CLOSURE across three repetitions with different libraries of modules. 
``Individual'' denotes that a module is assigned to a single sub-task. ``Semantic group'' and ``Random group'' denote that a module is assigned to a sub-task group including sub-tasks that are semantically similar or randomly selected. ``Order'' denotes that a module is selected by the order of a sub-task in a given program.
}
\label{table:results_modularity}
\centering
\begin{tabular}{l|c|c|cc}
\toprule
Library & The number & Specialization & \multicolumn{1}{c|}{CLEVR} & CLOSURE \\ %\cmidrule{2-5}
                        of modules & of modules & of modules & \multicolumn{1}{c|}{(In-Distribution)} & (Syst. Generalization) \\ \midrule
Individual & 26 & $\checkmark$ & \multicolumn{1}{l|}{98.0 $\pm$ 0.030} & 90.9 $\pm$ 0.49  \\
Semantic group & 12 & $\checkmark$ & \multicolumn{1}{l|}{98.1 $\pm$ 0.014} & \textbf{93.7  $\pm$ 0.55} \\ 
Random group & 12 & $\checkmark$ & \multicolumn{1}{l|}{97.9 $\pm$ 0.059} & 93.0  $\pm$ 0.29 \\ 
Order & 12 & & \multicolumn{1}{l|}{92.2 $\pm$ 1.5} & 68.4 $\pm$ 1.8   \\ \bottomrule 
\end{tabular}
\end{table}

%\input{neurips_2022/tabletest1}

\begin{table}[!t]
\caption{\emph{Ablation analysis.} Mean and standard deviation of accuracy (\%) on CLEVR and CLOSURE across three repetitions. We add imitations of properties of TMN, i.e., Variable number of  layers (VL) and Split tokens (ST) to the standard Transformer w/ PR. VL is an imitation of the question-specific composition of modules in TMN and changes the number of layers depending on a program length (up to $26$), but the each layer (module in TMN) is not specialized for specific sub-tasks. SoM stands for the specialization of the modules.}
\label{table:results_ablation}
\centering
\begin{tabular}{l|c|c|c|c|c}
\toprule
\multirow{2}{*}{Methods} &\multicolumn{3}{c|}{Properties} & CLEVR & CLOSURE \\ %\cmidrule{1-3}
 & VL & ST & SoM & (In-Distribution) & (Syst. Generalization) \\ \midrule
Transformer w/ PR & & & & \multicolumn{1}{l|}{97.1 $\pm$ 0.14} & 64.5 $\pm$ 2.5  \\
% Transformer w/ PR + DL & $\checkmark$ & & &\multicolumn{1}{l|}{97.0 $\pm$ 0.32} & 60.4  $\pm$ 2.7 \\
Transformer w/ PR + VL & $\checkmark$ & & &\multicolumn{1}{l|}{94.0 $\pm$ 1.8} & 60.2  $\pm$ 2.9 \\ 
% Transformer w/ PR + DL + ST& $\checkmark$ & $\checkmark$ &  & \multicolumn{1}{l|}{59.3 $\pm$ 0.50} &
Transformer w/ PR + VL + ST& $\checkmark$ & $\checkmark$ &  & \multicolumn{1}{l|}{56.8 $\pm$ 0.042} & 43.6 $\pm$ 0.59  \\
TMN-Stack & $\checkmark$ & $\checkmark$ & $\checkmark$ & \multicolumn{1}{l|}{98.0 $\pm$ 0.030} & \textbf{90.9 $\pm$ 0.49}   \\ \bottomrule
\end{tabular}
\end{table}
%\input{neurips_2022/tabletest2}

\subsection{Analysis} %Effect of Specialization of Modules}


\noindent
{\bf \color{blue}  Module Behaviors.}\quad
{\color{blue} We analyze the behaviors of our trained modules, i.e.,  how Transformer modules work, by visualizing attention maps (See Fig. \ref{figure:attentiom_map} in Appendix \ref{app:visualize}). The results indicate that the modules learn their functions properly.}

%\paragraph{Module Specialization.} 
\noindent
{\bf  Module Specialization.}\quad
While the question-specific composition of the modules is a key property of NMN, a recent work reports that a degree of modularity of the NMN also has large influence on systematic generalization \cite{vanessa}. Here we also investigate it. 
%how the degree of modularity affects the systematic generalization performance of the TMN-Stack. 
Table \ref{table:results_modularity} shows the mean accuracy of TMN-Stack with four different libraries of modules with different degree of modularity. The modules are composed depending on the question in every case, but the ways to assign the modules to sub-tasks, i.e., the specialization of the modules, are different. 
``Individual'' denotes that a module is assigned to a single sub-task ($26$ sub-tasks defined in CLEVR in total). This is the library used in the previous sections. 
``Semantic group'' denotes that a module is assigned to a sub-task group that includes semantically similar ones (e.g., {\tt FILTER\_COLOR}, {\tt FILTER\_SIZE}, ...). 
``Random group'' denotes that a module is assigned to a sub-task group that includes randomly selected ones (e.g., {\tt FILTER\_COLOR}, {\tt COUNT}, ...). 
``Order'' denotes that a module $m_i$ is selected by the order of a sub-task in a given program. The index of the selected module, $i$, is computed by $i=n\bmod M$, where $n$ is the order of the sub-task in the program and $M$ is the number of modules in the library (e.g., when $M=12$, 11th sub-task is assigned to $m_{11}$, 12th sub-task to $m_{0}$, ...). Unlike the other libraries, in this library the modules are not specialized for specific sub-tasks. See Appendix \ref{sec:libraries_appendix} for further details about each library. 
% All libraries are trained for 20 epochs on CLEVR dataset.

The result shows that the accuracy largely drops when the modules are not specialized even if the number of modules is the same (compare ``Order'' with ``Semantic group'' and ``Random group''). The degree of modularity (Individual vs Semantic group) and how sub-tasks are grouped (Semantic vs Random) also affects the systematic generalization performance. These results suggest that question-specific composition of modules is not enough and specialization of modules is also crucial. 


\noindent
{\bf Ablation Analysis.}
To further investigate whether the performance improvement by TMNs is gained from a combination of the question-specific composition and the module specialization or other properties, we add imitations of properties of TMN, i.e., Variable number of layers (VL) and Split tokens (ST) to the standard Transformer w/ PR. These are introduced in the following and then we report the results.

The standard Transformer w/ PR has a fixed number of encoder layers and it can be a reason to struggle with operating the novel combinations of the sub-tasks in a program as shown in Table \ref{table:results_all}. This result raises the question of whether the model can easily operate the sub-tasks only by changing the number of encoder layers depending on the program length. 
To investigate this question, we add a property named Variable number of layers (VL) to the Transformer w/ PR. With the VL, the model uses as many encoder layers as the program length (e.g., 18 layers are used to output an answer for an input program with a length of 18). VL can be regarded as an imitation of the question-specific  compositions of the modules in TMN, but each layer is not specialized for  specific sub-tasks. 

Each module of TMN takes only tokens for a sub-task as an input with visual features, while every layer of standard Transformer takes all input tokens in the program. Splitting the input tokens may help the model to understand the operation they should conduct at each layer. To investigate this question, we add this property as Split tokens (ST) to the Transformer w/ PR.

Table \ref{table:results_ablation} shows that any of the aforementioned properties do not improve the systematic generalization performance without the specialization of modules to sub-tasks (SoM). 
% , where all methods are trained for 20 epochs with CLEVR dataset. 
Even with Split tokens, the performance does not improve because the layers can not be specialized and splitting the token can spoil the flexibly of the standard Transformer.

%All methods are trained for 20 epochs with CLEVR dataset. 

% Dynamic layers is a imitation of dynamic composition of TMN, but each layers are not specialized for the specific sub-task like Order in \ref{table:results_modularity}. This could be a reason not to show the performance improvement. Even With Split tokens, the performance does not improve because the layers can not be specialized.

% Dynamic layers is a imitation of dynamic composition of TMN, but each layers are not specialized for the specific sub-task like Order in \ref{table:results_modularity}. This could be a reason not to show the performance improvement. 
% We add imitations of features of TMN to standard Transformer w/ PR to analyze the components of TMN, i.e., Dynamic layers and Split tokens. 



% Just write down:
% \begin{enumerate}
%   \item Modules are designed by human not automatically, self-modularization, self-supervised learning with large amount of data
%   \item Need programs or decomposing questions into sub-tasks (modules), or difficulty to apply to other datasets/tasks without programs
%   \item The number of layers of module are constant across all modules and it is practically decided, the number of layers can be optimized for each module
% \end{enumerate}

\begin{table}[!t]
\caption{\emph{Effect of pre-training.} Mean accuracy (\%) on CLEVR-CoGenT validation condition B and CLOSURE with two different feature extractors, which are an object detector pre-trained on Visual Genome (VG) and a ResNet-101 (without pre-training on VG).} 
\label{table:cogent_pretrain}
\centering
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c|}{CLEVR-CoGenT} & \multicolumn{3}{c}{CLOSURE}  \\ \cmidrule{2-7}
& w/o VG & w/ VG & $\Delta$ & w/o VG & w/ VG & $\Delta$ \\ \midrule %\hline
Transformer & 78.9 & 87.5 & 8.6 & 57.4 & 62.1 & 4.7 \\  %\hline
Transformer w/ PR & \textbf{81.7} & \textbf{88.7} & 6.9 & 64.5 & 64.5 & 0.005  \\  %\hline 
TMN-Stack (ours) & 80.6 & 86.9 & 6.3 & 90.9 & 92.7 & 1.7 \\  %\hline
TMN-Tree (ours) & 80.1 & 86.4 & 6.4 & \textbf{95.4} & \textbf{96.4} & 1.0    \\
\bottomrule
\end{tabular}
\end{table}

% \paragraph{Pre-training.}Furthermore, we investigate the effect of the pre-training of the networks and carefully control it in order to ensure a fair evaluation of systematic generalization. See Appendix \ref{sec:pretraining_appendix} for further details.

%\paragraph{Pre-training.} 
\noindent
{\bf Pre-training.}\quad
We investigate how the additional image data from other domains affects systematic generalization to novel combinations of visual attributes or linguistic constructs, i.e., CLEVR-CoGenT and CLOSURE, respectively. Table \ref{table:cogent_pretrain} shows the mean accuracy with two different visual features, namely, regional features extracted by an object detector pre-trained on Visual Genome (VG) and grid features extracted by a ResNet-101 without pre-training on VG. Across all the tested models, we observe that the performance gains from pre-training the visual feature extractor are  larger  for generalization to novel visual combinations and smaller for novel linguistic combinations.  
This highlights the need to control  pre-training in order to ensure a fair comparison of different methods for systematic generalization.
See Appendix \ref{sec:regional_appendix} and \ref{sec:pretraining_appendix} for further experiments.
